KAHANI: Culturally-Nuanced Visual Storytelling Tool for Non-Western Cultures

Large Language Models (LLMs) and Text-To-Image (T2I) models have demonstrated the ability to generate compelling text and visual stories. However, their outputs are predominantly aligned with the sensibilities of the Global North, often resulting in an outsider's gaze on other cultures. As a result, non-Western communities have to put extra effort into generating culturally specific stories. To address this challenge, we developed a visual storytelling tool called Kahani that generates culturally grounded visual stories for non-Western cultures. Our tool leverages off-the-shelf models GPT-4 Turbo and Stable Diffusion XL (SDXL). By using Chain of Thought (CoT) and T2I prompting techniques, we capture the cultural context from user's prompt and generate vivid descriptions of the characters and scene compositions. To evaluate the effectiveness of Kahani, we conducted a comparative user study with ChatGPT-4 (with DALL-E3) in which participants from different regions of India compared the cultural relevance of stories generated by the two tools. The results of the qualitative and quantitative analysis performed in the user study show that Kahani's visual stories are more culturally nuanced than those generated by ChatGPT-4. In 27 out of 36 comparisons, Kahani outperformed or was on par with ChatGPT-4, effectively capturing cultural nuances and incorporating more Culturally Specific Items (CSI), validating its ability to generate culturally grounded visual stories.

==> content/8-limitations.tex <==
\bheading{Limitations}

While we believe our study offers important insights into cultural story generation and evaluation, it has a few limitations.
\begin{itemize}
    \item To keep the study time-bound, we did not generate stories and visuals with participants in real-time, leaving the researchers as arbiters of the displayed content.
    \item Although both Kahani and ChatGPT are multi-turn tools, we only evaluated their first outputs, missing the opportunity to explore their abilities to handle iterative feedback or specific editing prompts—an aspect that could provide deeper insights into how each tool responds to evolving themes or cultural nuances.
    \item  Our comparative analysis was limited to ChatGPT; expanding the study to include other popular tools would provide a broader understanding of how different models handle cultural knowledge.
    \item Since our work primarily focused on incorporating cultural nuances in images, much focus was not given for character consistency while generating visual stories. 
\end{itemize}



